How to end password reuse on the web

We present a framework by which websites can coordinate to make it difficult for users to set similar passwords at these websites, in an effort to break the culture of password reuse on the web today. Though the design of such a framework is fraught with risks to users' security and privacy, we show that these risks can be effectively mitigated through careful scoping of the goals for such a framework and through principled design. At the core of our framework is a private set-membership-test protocol that enables one website to determine, upon a user setting a password for use at it, whether that user has already set a similar password at another participating website, but with neither side disclosing to the other the password(s) it employs in the protocol. Our framework then layers over this protocol a collection of techniques to mitigate the leakage necessitated by such a test. We verify via probabilistic model checking that these techniques are effective in maintaining account security, and since these mechanisms are consistent with common user experience today, our framework should be unobtrusive to users who do not reuse similar passwords across websites (e.g., due to having adopted a password manager). Through a working implementation of our framework and optimization of its parameters based on insights of how passwords tend to be reused, we show that our design can meet the scalability challenges facing such a service.

==> figures/non-tor/CDF.tex <==
% This file was created by matplotlib2tikz v0.6.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.129411764705882,0.380392156862745,0.549019607843137}

\pgfplotsset{every axis/.append style={
					xlabel={Response time (s)},
					ylabel={Proportion of responses},
					compat=1.3,
                    label style={font=\small},
                    tick label style={font=\small}  
                    }}

\begin{axis}[
%xmin=-0.334145424, xmax=19,
xmin=-1.03989173, xmax=20,
ymin=0, ymax=1,
width=\figurewidth,
height=\figureheight,
xtick={0,10,20},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
tick align=outside,
tick pos=left,
xmajorgrids,
minor tick num=1,
x grid style={lightgray!92.026143790849673!black},
ymajorgrids,
y grid style={lightgray!92.026143790849673!black},
%legend entries={{\nmbrSimilarPasswords = $2^7$},{\nmbrSimilarPasswords = $2^8$},{\nmbrSimilarPasswords = $2^9$},{\nmbrSimilarPasswords = $2^{10}$},{\nmbrSimilarPasswords = $2^{11}$},{\nmbrSimilarPasswords = $2^{12}$}},
%legend cell align={left},
%legend style={at={(0.97,0.03)}, anchor=south east, draw=white!80.0!black, nodes={scale=0.618, transform shape}}
]
%\addlegendimage{line width=1pt, densely dotted, color0}
%\addlegendimage{line width=1pt, dashed, color0}
%\addlegendimage{line width=1pt, dash pattern=on 1pt off 3pt on 3pt off 3pt, color0}
%\addlegendimage{line width=2pt, densely dotted, color0}
%\addlegendimage{line width=2pt, dashed, color0}
%\addlegendimage{line width=2pt, dash pattern=on 1pt off 3pt on 3pt off 3pt, color0}
\addplot [line width=1pt, color0, densely dotted]
table {%
0.27349974 0.015625
0.28442536 0.03125
0.289224 0.046875
0.29311378 0.0625
0.2966264 0.078125
0.30045682 0.09375
0.30302262 0.109375
0.30572774 0.125
0.30848328 0.140625
0.3104983 0.15625
0.3126841 0.171875
0.31417844 0.1875
0.31621744 0.203125
0.31792832 0.21875
0.31963498 0.234375
0.32082808 0.25
0.32238744 0.265625
0.32384262 0.28125
0.32546444 0.296875
0.32725484 0.3125
0.32837684 0.328125
0.32975192 0.34375
0.33101392 0.359375
0.33205448 0.375
0.3330951 0.390625
0.33420572 0.40625
0.33522814 0.421875
0.33613402 0.4375
0.33747252 0.453125
0.33864208 0.46875
0.33998504 0.484375
0.34099384 0.5
0.34206538 0.515625
0.34324266 0.53125
0.34442568 0.546875
0.3459943 0.5625
0.34766716 0.578125
0.34868214 0.59375
0.35023148 0.609375
0.35178158 0.625
0.35361428 0.640625
0.35541788 0.65625
0.35696326 0.671875
0.35968108 0.6875
0.36187258 0.703125
0.36390664 0.71875
0.36557888 0.734375
0.3682457 0.75
0.37088232 0.765625
0.3732217 0.78125
0.37555734 0.796875
0.37760558 0.8125
0.38144816 0.828125
0.38406894 0.84375
0.38630248 0.859375
0.38869674 0.875
0.39135532 0.890625
0.39329076 0.90625
0.39560746 0.921875
0.39794174 0.9375
0.40026112 0.953125
0.40385854 0.96875
0.4072463 0.984375
0.41619486 1
};
\addplot [line width=1pt, color0, dashed]
table {%
0.55985246 0.015625
0.57532978 0.03125
0.58442552 0.046875
0.59265792 0.0625
0.59917448 0.078125
0.6055718 0.09375
0.61048768 0.109375
0.61620962 0.125
0.61970412 0.140625
0.62235522 0.15625
0.62650682 0.171875
0.63009432 0.1875
0.63361704 0.203125
0.63638382 0.21875
0.63903202 0.234375
0.64130356 0.25
0.64504434 0.265625
0.64802702 0.28125
0.65039554 0.296875
0.65265332 0.3125
0.6549896 0.328125
0.65759788 0.34375
0.6596515 0.359375
0.66153756 0.375
0.6638372 0.390625
0.66564706 0.40625
0.66722758 0.421875
0.66926878 0.4375
0.6715653 0.453125
0.67347938 0.46875
0.67503616 0.484375
0.67722722 0.5
0.67870016 0.515625
0.68038058 0.53125
0.68184666 0.546875
0.68381978 0.5625
0.68558852 0.578125
0.68801226 0.59375
0.69039072 0.609375
0.69238048 0.625
0.69492336 0.640625
0.69809176 0.65625
0.70108542 0.671875
0.70374992 0.6875
0.70610614 0.703125
0.70901888 0.71875
0.7135845 0.734375
0.71765462 0.75
0.72136958 0.765625
0.7254412 0.78125
0.731164 0.796875
0.73623712 0.8125
0.74274296 0.828125
0.75081744 0.84375
0.75767432 0.859375
0.7634746 0.875
0.7679827 0.890625
0.77241106 0.90625
0.77760154 0.921875
0.78261196 0.9375
0.78688692 0.953125
0.79107062 0.96875
0.79648708 0.984375
0.80599142 1
};
\addplot [line width=1pt, color0, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
1.15035338 0.015625
1.17787422 0.03125
1.19517512 0.046875
1.2107521 0.0625
1.222919 0.078125
1.23412308 0.09375
1.24378852 0.109375
1.25115104 0.125
1.25968412 0.140625
1.26768636 0.15625
1.27389196 0.171875
1.27942888 0.1875
1.28456288 0.203125
1.29094758 0.21875
1.29549368 0.234375
1.2998503 0.25
1.30479656 0.265625
1.30950336 0.28125
1.313475 0.296875
1.31744342 0.3125
1.32289818 0.328125
1.32803986 0.34375
1.3315931 0.359375
1.3362899 0.375
1.33997484 0.390625
1.34280298 0.40625
1.34660868 0.421875
1.3500979 0.4375
1.35284868 0.453125
1.35555226 0.46875
1.35830298 0.484375
1.3607046 0.5
1.36367356 0.515625
1.36684342 0.53125
1.3703859 0.546875
1.37375566 0.5625
1.37673958 0.578125
1.3794009 0.59375
1.3825342 0.609375
1.38529676 0.625
1.38831368 0.640625
1.39336862 0.65625
1.39690582 0.671875
1.40112336 0.6875
1.4045739 0.703125
1.40929342 0.71875
1.41355258 0.734375
1.41853856 0.75
1.42285058 0.765625
1.42829848 0.78125
1.43490244 0.796875
1.440771 0.8125
1.44723548 0.828125
1.4569013 0.84375
1.47277312 0.859375
1.48881616 0.875
1.50567984 0.890625
1.5255597 0.90625
1.5395784 0.921875
1.5537162 0.9375
1.57359602 0.953125
1.59202686 0.96875
1.6067854 0.984375
1.62697456 1
};
\addplot [line width=2pt, color0, densely dotted]
table {%
2.265376 0.015625
2.33250606 0.03125
2.36567332 0.046875
2.39854488 0.0625
2.42753028 0.078125
2.45223974 0.09375
2.47193204 0.109375
2.49107118 0.125
2.50363094 0.140625
2.51780584 0.15625
2.5372247 0.171875
2.54751284 0.1875
2.55905068 0.203125
2.56860274 0.21875
2.57934312 0.234375
2.58670918 0.25
2.59373464 0.265625
2.60075748 0.28125
2.60959086 0.296875
2.61810152 0.3125
2.6274025 0.328125
2.63364554 0.34375
2.6428975 0.359375
2.650818 0.375
2.6586682 0.390625
2.66663402 0.40625
2.6745711 0.421875
2.67979378 0.4375
2.68591132 0.453125
2.69137538 0.46875
2.69736902 0.484375
2.70326326 0.5
2.70939274 0.515625
2.7143173 0.53125
2.71917928 0.546875
2.72517924 0.5625
2.7295833 0.578125
2.73414044 0.59375
2.73913342 0.609375
2.74351636 0.625
2.7483367 0.640625
2.75337562 0.65625
2.76053538 0.671875
2.76739532 0.6875
2.77462114 0.703125
2.78081736 0.71875
2.78762462 0.734375
2.7951385 0.75
2.80450742 0.765625
2.81222166 0.78125
2.82399356 0.796875
2.83481958 0.8125
2.84538888 0.828125
2.8583559 0.84375
2.8776413 0.859375
2.89842828 0.875
2.92628078 0.890625
2.95951176 0.90625
3.01090368 0.921875
3.05174876 0.9375
3.08594896 0.953125
3.1375835 0.96875
3.17835414 0.984375
3.21709172 1
};
\addplot [line width=2pt, color0, dashed]
table {%
4.58357376 0.015625
4.67661592 0.03125
4.7288604 0.046875
4.7895065 0.0625
4.8507511 0.078125
4.89480166 0.09375
4.93298338 0.109375
4.96071982 0.125
4.98656546 0.140625
5.01862174 0.15625
5.0432963 0.171875
5.06636238 0.1875
5.09093274 0.203125
5.11011446 0.21875
5.12787136 0.234375
5.14325368 0.25
5.15673672 0.265625
5.17151986 0.28125
5.19088834 0.296875
5.20569884 0.3125
5.22114142 0.328125
5.2359948 0.34375
5.2493319 0.359375
5.26283508 0.375
5.2720575 0.390625
5.2855647 0.40625
5.29620286 0.421875
5.30779092 0.4375
5.31936578 0.453125
5.32960544 0.46875
5.33837222 0.484375
5.3472185 0.5
5.3592606 0.515625
5.3715285 0.53125
5.38057456 0.546875
5.3925043 0.5625
5.4016486 0.578125
5.40872312 0.59375
5.4165254 0.609375
5.4223165 0.625
5.43163738 0.640625
5.43854184 0.65625
5.44792142 0.671875
5.4569467 0.6875
5.46374594 0.703125
5.47237426 0.71875
5.47937842 0.734375
5.48910696 0.75
5.49681016 0.765625
5.50608908 0.78125
5.51694032 0.796875
5.52918348 0.8125
5.5442121 0.828125
5.56065186 0.84375
5.576958 0.859375
5.5974509 0.875
5.62259166 0.890625
5.65602744 0.90625
5.69606788 0.921875
5.73250596 0.9375
5.78730182 0.953125
5.86549898 0.96875
6.01115242 0.984375
6.21751328 1
};
\addplot [line width=2pt, color0, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
9.44818264 0.015625
9.62039346 0.03125
9.76181954 0.046875
9.90140282 0.0625
10.01314494 0.078125
10.08772276 0.09375
10.16518852 0.109375
10.20742354 0.125
10.28282088 0.140625
10.33639752 0.15625
10.37758336 0.171875
10.41428862 0.1875
10.44338464 0.203125
10.49019826 0.21875
10.52076818 0.234375
10.55445076 0.25
10.58196734 0.265625
10.62087536 0.28125
10.64792046 0.296875
10.67791738 0.3125
10.70173278 0.328125
10.73085404 0.34375
10.74438398 0.359375
10.7670112 0.375
10.7854286 0.390625
10.8149285 0.40625
10.83872686 0.421875
10.85789974 0.4375
10.8785348 0.453125
10.8929971 0.46875
10.91268898 0.484375
10.92878852 0.5
10.94382694 0.515625
10.95664696 0.53125
10.9698144 0.546875
10.98655254 0.5625
10.99913844 0.578125
11.00949182 0.59375
11.02187848 0.609375
11.04056328 0.625
11.05184878 0.640625
11.0628288 0.65625
11.0756224 0.671875
11.08922252 0.6875
11.10320564 0.703125
11.11649986 0.71875
11.12778102 0.734375
11.14114804 0.75
11.1517115 0.765625
11.17033622 0.78125
11.1843915 0.796875
11.20178606 0.8125
11.22026124 0.828125
11.23877224 0.84375
11.26269214 0.859375
11.2935318 0.875
11.32404994 0.890625
11.37329852 0.90625
11.42499604 0.921875
11.49013752 0.9375
11.5565612 0.953125
11.67272208 0.96875
11.92200338 0.984375
12.42640302 1
};

\end{axis}

\end{tikzpicture}

==> figures/tor/tor_CDF.tex <==
% This file was created by matplotlib2tikz v0.6.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.129411764705882,0.380392156862745,0.549019607843137}

\pgfplotsset{every axis/.append style={
					xlabel={Response time (s)},
%					ylabel={Proportion of responses (\#=64)},
%					ylabel={                               },
					compat=1.3,
                    label style={font=\small},
                    tick label style={font=\small}  
                    }}

\begin{axis}[
xmin=-1.03989173, xmax=40,
ymin=0, ymax=1,
width=\figurewidth,
height=\figureheight,
tick align=outside,
tick pos=left,
xtick={0,10,20,30,40},
xticklabels={0,10,20,30,40},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={},
%yticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
minor tick num=1,
xmajorgrids,
x grid style={lightgray!92.026143790849673!black},
ymajorgrids,
y grid style={lightgray!92.026143790849673!black},
%legend entries={{\nmbrSimilarPasswords = $2^7$},{\nmbrSimilarPasswords = $2^8$},{\nmbrSimilarPasswords = $2^9$},{\nmbrSimilarPasswords = $2^{10}$},{\nmbrSimilarPasswords = $2^{11}$},{\nmbrSimilarPasswords = $2^{12}$}},
%legend cell align={left},
%legend style={at={(0.97,0.03)}, anchor=south east, draw=white!80.0!black, nodes={scale=0.618, transform shape}}
]
%\addlegendimage{line width=1pt, densely dotted, color0}
%\addlegendimage{line width=1pt, dashed, color0}
%\addlegendimage{line width=1pt, dash pattern=on 1pt off 3pt on 3pt off 3pt, color0}
%\addlegendimage{line width=2pt, densely dotted, color0}
%\addlegendimage{line width=2pt, dashed, color0}
%\addlegendimage{line width=2pt, dash pattern=on 1pt off 3pt on 3pt off 3pt, color0}
\addplot [line width=1pt, densely dotted, color0]
table {%
0.36183018 0.015625
0.38433716 0.03125
0.39640944 0.046875
0.40425282 0.0625
0.41144338 0.078125
0.41785148 0.09375
0.42452374 0.109375
0.42949778 0.125
0.43436482 0.140625
0.44123794 0.15625
0.45133744 0.171875
0.46219234 0.1875
0.47267654 0.203125
0.48601552 0.21875
0.5009961 0.234375
0.52872674 0.25
0.65562518 0.265625
0.69595766 0.28125
0.72401264 0.296875
0.74355304 0.3125
0.76009358 0.328125
0.7758206 0.34375
0.78852062 0.359375
0.80369498 0.375
0.8146351 0.390625
0.82582636 0.40625
0.83960598 0.421875
0.8560281 0.4375
0.8664615 0.453125
0.8799361 0.46875
0.89135824 0.484375
0.9052808 0.5
0.91592276 0.515625
0.92860992 0.53125
0.94152586 0.546875
0.9499229 0.5625
0.95752752 0.578125
0.96693568 0.59375
0.97668378 0.609375
0.98837142 0.625
1.00124438 0.640625
1.0115567 0.65625
1.0196832 0.671875
1.02891302 0.6875
1.04312866 0.703125
1.05342572 0.71875
1.06916312 0.734375
1.0872616 0.75
1.10278712 0.765625
1.1208045 0.78125
1.1470801 0.796875
1.1775404 0.8125
1.24462798 0.828125
1.3046589 0.84375
1.35190578 0.859375
1.3809334 0.875
1.4127208 0.890625
1.45082456 0.90625
1.47833642 0.921875
1.52544198 0.9375
1.5858763 0.953125
1.6485246 0.96875
1.70524622 0.984375
1.76314662 1
};
\addplot [line width=1pt, dashed, color0]
table {%
0.70363294 0.015625
0.73098826 0.03125
0.74985932 0.046875
0.7655484 0.0625
0.77669904 0.078125
0.78948728 0.09375
0.80442396 0.109375
0.81594452 0.125
0.83011208 0.140625
0.84402422 0.15625
0.85606002 0.171875
0.86731996 0.1875
0.88239048 0.203125
0.89418014 0.21875
0.91153698 0.234375
0.94387872 0.25
1.18056236 0.265625
1.22529836 0.28125
1.26417248 0.296875
1.2929663 0.3125
1.30790462 0.328125
1.32780778 0.34375
1.34884872 0.359375
1.36566114 0.375
1.37951118 0.390625
1.39570616 0.40625
1.41014268 0.421875
1.42632196 0.4375
1.444556 0.453125
1.4603441 0.46875
1.473952 0.484375
1.48346892 0.5
1.49780156 0.515625
1.50959084 0.53125
1.52384538 0.546875
1.54137176 0.5625
1.55828468 0.578125
1.57427116 0.59375
1.59306738 0.609375
1.6108463 0.625
1.6333609 0.640625
1.6548365 0.65625
1.67940314 0.671875
1.7028242 0.6875
1.72424002 0.703125
1.74324536 0.71875
1.76439458 0.734375
1.78549256 0.75
1.8062104 0.765625
1.8224327 0.78125
1.84681942 0.796875
1.87737564 0.8125
1.9645958 0.828125
2.0147829 0.84375
2.06150974 0.859375
2.11992484 0.875
2.17120286 0.890625
2.24047806 0.90625
2.32091308 0.921875
2.37470616 0.9375
2.40839366 0.953125
2.45306738 0.96875
2.49226192 0.984375
2.55862662 1
};
\addplot [line width=1pt, dash pattern=on 1pt off 3pt on 3pt off 3pt, color0]
table {%
1.63225446 0.015625
1.70362722 0.03125
1.74744826 0.046875
1.79127194 0.0625
1.81795326 0.078125
1.84431798 0.09375
1.86447042 0.109375
1.88446856 0.125
1.9065299 0.140625
1.92739768 0.15625
1.9414087 0.171875
1.96530242 0.1875
1.98013504 0.203125
1.99591992 0.21875
2.02451952 0.234375
2.06364644 0.25
2.30070048 0.265625
2.35418782 0.28125
2.38780634 0.296875
2.40603768 0.3125
2.4208577 0.328125
2.43956058 0.34375
2.45286824 0.359375
2.46440658 0.375
2.47954658 0.390625
2.4943765 0.40625
2.51328816 0.421875
2.53035788 0.4375
2.54479932 0.453125
2.559237 0.46875
2.58600946 0.484375
2.59835474 0.5
2.6146662 0.515625
2.63391982 0.53125
2.65634204 0.546875
2.6827731 0.5625
2.72018506 0.578125
2.76234102 0.59375
2.86677524 0.609375
2.96239622 0.625
3.09918838 0.640625
3.1660029 0.65625
3.20985452 0.671875
3.27463152 0.6875
3.3013574 0.703125
3.32656042 0.71875
3.34728214 0.734375
3.36755576 0.75
3.38582372 0.765625
3.40156996 0.78125
3.42145514 0.796875
3.43501324 0.8125
3.4595409 0.828125
3.48977318 0.84375
3.51788918 0.859375
3.54612926 0.875
3.5745418 0.890625
3.61068568 0.90625
3.66628064 0.921875
3.79320546 0.9375
4.01980234 0.953125
4.13337148 0.96875
4.21337354 0.984375
4.30172164 1
};
\addplot [line width=2pt, densely dotted, color0]
table {%
3.70934404 0.015625
3.79974486 0.03125
3.85838258 0.046875
3.90094952 0.0625
3.94260032 0.078125
3.9800199 0.09375
4.0206518 0.109375
4.05484396 0.125
4.08958 0.140625
4.11391846 0.15625
4.14733602 0.171875
4.16878658 0.1875
4.19671492 0.203125
4.22383418 0.21875
4.25946484 0.234375
4.32826688 0.25
4.86088388 0.265625
4.90163372 0.28125
4.93596442 0.296875
4.96740574 0.3125
4.9924555 0.328125
5.0224495 0.34375
5.06342398 0.359375
5.08939634 0.375
5.11612592 0.390625
5.14524188 0.40625
5.17900012 0.421875
5.21128014 0.4375
5.24799334 0.453125
5.28065606 0.46875
5.31910334 0.484375
5.34724308 0.5
5.3832183 0.515625
5.41273204 0.53125
5.4470362 0.546875
5.49389046 0.5625
5.56060208 0.578125
5.67639064 0.59375
5.84335974 0.609375
6.04997928 0.625
6.11514 0.640625
6.16244042 0.65625
6.20289142 0.671875
6.2341063 0.6875
6.25950824 0.703125
6.28832666 0.71875
6.32246072 0.734375
6.34641076 0.75
6.36989502 0.765625
6.38719794 0.78125
6.40355634 0.796875
6.42365358 0.8125
6.44204404 0.828125
6.4615016 0.84375
6.48073566 0.859375
6.5010187 0.875
6.52530866 0.890625
6.57787466 0.90625
6.76201464 0.921875
7.00346036 0.9375
7.15129206 0.953125
7.27858932 0.96875
7.42646322 0.984375
7.56088032 1
};
\addplot [line width=2pt, dashed, color0]
table {%
8.33237102 0.015625
8.43967714 0.03125
8.49846158 0.046875
8.56332812 0.0625
8.6210496 0.078125
8.69505948 0.09375
8.75140822 0.109375
8.809419 0.125
8.8656268 0.140625
8.9155365 0.15625
8.95627956 0.171875
9.01472102 0.1875
9.0593899 0.203125
9.11402722 0.21875
9.17644068 0.234375
9.28433544 0.25
10.00684456 0.265625
10.09581272 0.28125
10.15623164 0.296875
10.22224536 0.3125
10.2761637 0.328125
10.31629394 0.34375
10.3744757 0.359375
10.445035 0.375
10.5193079 0.390625
10.5772489 0.40625
10.65757318 0.421875
10.73544858 0.4375
10.78872876 0.453125
10.84115914 0.46875
10.89471272 0.484375
10.9744953 0.5
11.03773602 0.515625
11.08275758 0.53125
11.14991772 0.546875
11.22354698 0.5625
11.34039516 0.578125
11.58011376 0.59375
11.81738696 0.609375
11.97653038 0.625
12.07172292 0.640625
12.15967674 0.65625
12.22137866 0.671875
12.26832928 0.6875
12.3242546 0.703125
12.36649662 0.71875
12.4038858 0.734375
12.44264812 0.75
12.47461102 0.765625
12.5178684 0.78125
12.54902908 0.796875
12.58777422 0.8125
12.62316024 0.828125
12.66145292 0.84375
12.6987502 0.859375
12.73417816 0.875
12.78464988 0.890625
12.85180876 0.90625
12.99365858 0.921875
13.34668284 0.9375
13.54668842 0.953125
13.7299149 0.96875
13.8765818 0.984375
14.03544998 1
};
\addplot [line width=2pt, dash pattern=on 1pt off 3pt on 3pt off 3pt, color0]
table {%
17.21132336 0.015625
17.3958325 0.03125
17.54847588 0.046875
17.6974838 0.0625
17.86403452 0.078125
18.02667892 0.09375
18.56900064 0.109375
18.67036102 0.125
18.78689154 0.140625
18.89492 0.15625
18.98153832 0.171875
19.09127584 0.1875
19.1851178 0.203125
19.3135443 0.21875
19.43042522 0.234375
19.60717636 0.25
20.20469068 0.265625
20.44484972 0.28125
20.65179698 0.296875
20.77028894 0.3125
20.91004778 0.328125
21.01587246 0.34375
21.1634229 0.359375
21.28450624 0.375
21.43353644 0.390625
21.55812354 0.40625
21.67914162 0.421875
21.80268048 0.4375
21.9238068 0.453125
22.03822998 0.46875
22.15650546 0.484375
22.28888848 0.5
22.44449694 0.515625
22.60281182 0.53125
22.7781268 0.546875
22.96031744 0.5625
23.14535018 0.578125
23.59648604 0.59375
23.86263038 0.609375
24.10698218 0.625
24.30046844 0.640625
24.43842878 0.65625
24.54448136 0.671875
24.65225552 0.6875
24.74689476 0.703125
24.82850962 0.71875
24.9153817 0.734375
24.97923864 0.75
25.04755012 0.765625
25.130048 0.78125
25.20745738 0.796875
25.2737455 0.8125
25.35441264 0.828125
25.42803916 0.84375
25.61806214 0.859375
25.72082022 0.875
25.84465414 0.890625
26.12328494 0.90625
26.37238592 0.921875
26.8862743 0.9375
27.36057178 0.953125
27.66308058 0.96875
27.93953218 0.984375
28.39626838 1
};
\end{axis}

\end{tikzpicture}


==> figures/tor/tor_e2e_latency.tex <==
% This file was created by matplotlib2tikz v0.6.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.129411764705882,0.380392156862745,0.549019607843137}

\pgfplotsset{every axis/.append style={
					xlabel={Response time (\secs)},
%					ylabel={Proportion of responders (\#=64)},
					compat=1.3,
                    label style={font=\small},
                    tick label style={font=\small}  
                    }}

\begin{axis}[
xmin=-0.341182282, xmax=40,
ymin=0, ymax=1,
width=\figurewidth,
height=\figureheight,
tick align=outside,
tick pos=left,
minor tick num=1,
xtick={0,10,20,30,40},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={},
%yticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
xmajorgrids,
x grid style={lightgray!92.026143790849673!black},
ymajorgrids,
y grid style={lightgray!92.026143790849673!black},
%legend entries={{\nmbrSimilarPasswords = $2^7$},{\nmbrSimilarPasswords = $2^8$},{\nmbrSimilarPasswords = $2^9$},{\nmbrSimilarPasswords = $2^{10}$},{\nmbrSimilarPasswords = $2^{11}$},{\nmbrSimilarPasswords = $2^{12}$}},
%legend cell align={left},
%legend style={at={(0.97,0.03)}, anchor=south east, draw=white!80.0!black, nodes={scale=0.618, transform shape}}
]
%\addlegendimage{line width=1pt, densely dotted, color0}
%\addlegendimage{line width=1pt, dashed, color0}
%\addlegendimage{line width=1pt, dash pattern=on 1pt off 3pt on 3pt off 3pt, color0}
%\addlegendimage{line width=2pt, densely dotted, color0}
%\addlegendimage{line width=2pt, dashed, color0}
%\addlegendimage{line width=2pt, dash pattern=on 1pt off 3pt on 3pt off 3pt, color0}
\addplot [line width=1pt, densely dotted, color0]
table {%
1.48565376 0.015625
1.95511426 0.25
2.201871 0.5
2.82597838 0.75
3.3022177 1
};
\addplot [line width=1pt, dashed, color0]
table {%
2.3766118 0.015625
2.862802 0.25
3.2699948 0.5
3.72270524 0.75
4.66240986 1
};
\addplot [line width=1pt, dash pattern=on 1pt off 3pt on 3pt off 3pt, color0]
table {%
3.53786544 0.015625
4.20764612 0.25
5.4170094 0.5
5.73985296 0.75
6.7232246 1
};
\addplot [line width=2pt, densely dotted, color0]
table {%
6.13149926 0.015625
7.47828284 0.25
9.12166248 0.5
9.54902008 0.75
11.0877671 1
};
\addplot [line width=2pt, dashed, color0]
table {%
11.41012414 0.015625
13.72834182 0.25
16.736895 0.5
17.73859294 0.75
19.73507796 1
};
\addplot [line width=2pt, dash pattern=on 1pt off 3pt on 3pt off 3pt, color0]
table {%
22.91918708 0.015625
26.64385434 0.25
31.54082418 0.5
34.23714754 0.75
38.0223746 1
};
\end{axis}

\end{tikzpicture}


==> figures/tor/tor_resps.tex <==
% This file was created by matplotlib2tikz v0.6.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.129411764705882,0.380392156862745,0.549019607843137}

\pgfplotsset{every axis/.append style={
					xlabel={\nmbrSimilarPasswords},
%					ylabel={Protocol running time (s)},
					compat=1.3,
                    label style={font=\small},
                    tick label style={font=\small}  
                    }}

\begin{axis}[
xmin=128, xmax=4096,
ymin=0, ymax=60,
xmode=log,
log basis x={2},
xtick={128,256,512,1024,2048,4096},
ytick={0,10,20,30,40,50,60},
yticklabels={},
width=\figurewidth,
height=\figureheight,
tick align=outside,
tick pos=left,
minor tick num=1,
xmajorgrids,
x grid style={lightgray!92.026143790849673!black},
ymajorgrids,
y grid style={lightgray!92.026143790849673!black},
%legend entries={{1 responder},{32 responders},{64 responders},{96 responders},{128 responders}},
%legend cell align={left},
%legend style={at={(0.03,0.97)}, anchor=north west, draw=white!80.0!black, nodes={scale=0.55, transform shape}}
]
%\addlegendimage{line width=1pt, color0}
%\addlegendimage{line width=1pt, color0, dotted}
%\addlegendimage{line width=1pt, color0, dash pattern=on 1pt off 3pt on 3pt off 3pt}
%\addlegendimage{line width=1pt, color0, dashed}
%\addlegendimage{line width=2pt, color0, dashed}
\addplot [line width=1pt, color0]
table {%
128 1.80276424
256 2.67040142
512 4.49651676
1024 7.47617528
2048 13.1238372
4096 25.08883928
};
\addplot [line width=1pt, color0, dotted]
table {%
128 2.7080117
256 3.70559346
512 5.53991662
1024 9.39000844
2048 17.0989824
4096 33.26568904
};
\addplot [line width=1pt, color0, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
128 3.3022177
256 4.66240986
512 6.7232246
1024 11.0877671
2048 19.73507796
4096 38.0223746
};
\addplot [line width=1pt, color0, dashed]
table {%
128 3.42254084
256 4.69043296
512 7.05244956
1024 12.43998506
2048 22.71355764
4096 44.51036384
};
\addplot [line width=2pt, color0, dashed]
table {%
128 3.58230948
256 4.56667798
512 7.52800982
1024 13.6724325
2048 25.92064192
4096 50.80265902
};
\end{axis}

\end{tikzpicture}
